Towards Neural Network based Cognitive Models of Dynamic Decision-Making by Humans

Modeling human cognitive processes in dynamic decision-making tasks has been an endeavor in AI for a long time because such models can help make AI systems more intuitive, personalized, mitigate any human biases, and enhance training in simulation. Some initial work has attempted to utilize neural networks (and large language models) but often assumes one common model for all humans and aims to emulate human behavior in aggregate. However, the behavior of each human is distinct, heterogeneous, and relies on specific past experiences in certain tasks. For instance, consider two individuals responding to a phishing email: one who has previously encountered and identified similar threats may recognize it quickly, while another without such experience might fall for the scam. In this work, we build on Instance Based Learning (IBL) that posits that human decisions are based on similar situations encountered in the past. However, IBL relies on simple fixed form functions to capture the mapping from past situations to current decisions. To that end, we propose two new attention-based neural network models to have open form non-linear functions to model distinct and heterogeneous human decision-making in dynamic settings. We experiment with two distinct datasets gathered from human subject experiment data, one focusing on detection of phishing email by humans and another where humans act as attackers in a cybersecurity setting and decide on an attack option. We conducted extensive experiments with our two neural network models, IBL, and GPT3.5, and demonstrate that the neural network models outperform IBL significantly in representing human decision-making, while providing similar interpretability of human decisions as IBL. Overall, our work yields promising results for further use of neural networks in cognitive modeling of human decision making.

==> sections/1_intro.tex <==
\section{Introduction}

Since the early days of AI, cognitive approaches to AI have aimed to emulate human cognitive processes with the goal of designing computer agents that exhibit human like decision making~\citep{riedl2012interactive} and (possibly superior) intelligence~\citep{newell1994unified}. While recent advances in AI have relied on neural networks, the goal of making realistic human agents is still very relevant. Work in this space has built human like agents, particularly in game play~\citep{laird2001knows,miyashita2017developing,siu2021evaluation,asfour2023harnessing}. Prior approaches aim to replicate human decision making in the aggregate (e.g., have one model for all humans)  or within broad categories of human personalities (e.g., impulsive, cautious) or simple personalized models. However, human decision-making is complex and heterogeneous, which does not neatly fit into categories of personalities and simple closed form formulas might be inadequate to capture the complexities. The need for a high fidelity personalized model of observed humans' decision-making arises in many domains such as human detection of phishing email, understanding human attackers in cyber attacks, knowledge consumption in education settings, and many others. In the application of phishing, attacks rely on heterogeneity of decision-making, including human fallacies, to be successful. Developing realistic dynamic decision-making models of a particular human from \emph{observed past decisions} can lead to the development of personalized interventions that make humans better at detecting phishing emails. In this work, we aim to build high fidelity, fine-grained and data driven model of human behavior in dynamic decsion-making. 

We base our work on a popular cognitive model of human behavior, namely Instance Based Learning (IBL). IBL is an approach of modelling decisions from experience, developed
to explain human learning in dynamic decision environments~\cite{gonzalez2003instance}. IBL provides a decision-making algorithm that is guided by the
recognition and retrieval of past experiences (i.e., instances)
according to their similarity to a current decision situation.
An \emph{instance} in IBL is a memory unit consisting of three elements: a situation (set
of attributes that give a context to the decision, or state s); a
decision (the action taken); and a feedback (expected utility or
experienced outcome of the action taken in the situation). IBL model has been widely used in various contexts to model human behavior~\citep{gonzalez2003instance,cranford2021towards}; we aim to fuse ideas from IBL and the expressivity of neural networks  to model dynamic decision-making with high fidelity. Other prior works in human behavior modelling produce either one monolithic model~\citep{cheung2021attacker,thakoor2020exploiting} or aim to model generic behavior over many tasks~\citep{mao2023alympics,park2023generative}. In contrast, we aim to mimic diverse and possibly not rational behavior for some particular task.
%We also note that typically the data per human participant is not enough to build a separate neural network based model for each human participant in most datasets.

 We take inspiration from the IBL model to build two different attention based neural network based models for the above problem. Following IBL, the core idea in both these models is to personalize the model to each human by conditioning on the memory of the human; in this sense, we learn a mapping from past memory units, i.e., tuples of (situation, action, feedback), and the current situation to the next decision. We posit that the use of past decisions of a human in the conditioning makes the model aligned to the specific behavior of the particular human. Our first model Token-Level Personalized Memory Integrated Model (TL-PMIM) is based on fine-tuning a Large Language Model (LLM), namely Llama 7B, with the given limited dataset, that provides a highly expressive model but at the cost of interpretability. Our second hybrid model Instance-Level Personalized Memory Integrated Model (IL-PMIM) balances expressivity and interpretability by building a simple attention layer based model, where the attention weights can be directly interpreted. We also use GPT3.5 as yet another alternate model.

We conduct thorough experiments using data gathered in prior work from two separate human subject experiments: one experiment involved participants detecting phishing emails and another experiment involved participants acting as attackers in a cyber-security deception game. We analyze the results from IBL, TL-PMIM, IL-PMIM, and GPT3.5. We find that TL-PMIM best mimics individual human behavior. We also perform further fine-grained analysis showing that all models mimic better when the human participant is better at the underlying task, or in other words, mimicking sub-optimal behavior appears to be more challenging. We believe that this is due to less variability in behavior when tasks are performed successfully and more diverse kinds of mistakes (by the same human) when performing poor at a task. We also show that prior knowledge inbuilt in GPT may not always be beneficial in modelling a single human's behavior. Overall, we believe that our work at the intersection of behavioral science and AI will lead to open doors for further research in this area.

%\textbf{Problem Statement.} Given a dataset $D={(x_i,a_i)}_{i=1}^N$, we would like to learn a policy $\pi: \mathcal{X}\rightarrow\mathcal{A}$ that is close to the underlying pattern in the data. 

==> sections/2_related.tex <==
\section{Related Work}

There is a vast amount of literature on modelling human behavior in different areas of research~\citep{fuchs2023modeling,laird2022analysis,kahneman2002foundations}, which is not possible to describe in short. Instead, we focus on the applied problem domain that we study, starting with phishing email problem.

\textbf{Human Behavioral Modelling in Phishing Email Domain}:  Researchers have thoroughly investigated human behavior when tasked to identify a new (phishing or ham) email. Prior work has studied the factors that make a phishing email hard to be detected~\citep{singh2020makes}. Also, people have investigated the ways that can improve human's capability of detecting the phishing emails~\cite{}. Moreover, prior work has applied the instance-based learning (IBL) in modeling human's response to the emails from observed data~\citep{cranford2019modeling,xu2022modeling}. A recent work~\citep{asfour2023harnessing} has attempted to simulate human behavior response to phishing emails using LLMs by asking the LLM to simulate broad personality traits; this work is not data driven and does not provide a personalized modeling of a particular human (based on observed past decisions) and hence such work cannot be used for developing personalized interventions for training humans to detect emails. Prior work on interventions have also mostly relied on domain expert advice~\citep{sheng2009improving,kumaraguru2010teaching} rather than building a personalized model of human sub-optimality. 

Somewhat farther away, there are attack related work focusing on generating phishing emails by LLMs~\citep{hazell2023large,karanjai2022targeted,sharma2023well}, as well as defense related work proposing use of LLMs for detecting the phishing emails~\citep{heiding2023devising}.
Some works have build autonomous agent using LLMs with the memory components~\citep{mao2023alympics, park2023generative}. These works are designed to built more generic agents and study emergent behavior, unlike our goal of heterogeneous personalized models built from observed past decisions in a specific task. Even farther away, there is a vast literature on techniques to detect phishing email and many popular email provider use a variety of learning methods.

\textbf{Human Behavioral Modelling of Attackers in Cyber-security}: This is a relatively less explored research topic. Some research in this area has originated from behavioral game theory that explore beyond the rational model of human behavior~\citep{cheung2021attacker,thakoor2020exploiting} originating in Stackelberg security games~\citep{sinha2018stackelberg}. Recently, there have been applications of the IBL model in more realistic modeling of attacker behavior~\cite{cranford2021towards}. More broadly, work in physical security has explored different aspects of human behavior in games~\citep{kar2015game}.



==> sections/3_method.tex <==
\section{Behavioral Modeling with Memory Mechanism}

%To capture the personalities in human's behavior, we propose a framework that utilizes the personal memories and make predictions that is conditioned on the memory. Under the framework, we have shown two instances which use different base model as predictors. 
We describe all the different approaches that we compare in this work. We start with the known IBL model here in order to introduce terminology and concepts that help in describing the other new proposed models.

\subsection{IBL Model} 

In Instance Base Learning~\cite{gonzalez2003instance}, an action made by a human is modelled as occurring by activating memory instances of past experiences associated with each action/decision. A memory instance is a tuple $(s,a,u)$ denoting a situation (state) $s$ in which action/decision $a$ was taken resulting in outcome/utility of a scalar $u$. A state $s_i$ is represented by $K$ attributes, with $s_{i,k}$ denoting the $k$-th attribute. An action $a \in A$ belongs to a given set $A$. Memory is just a sequence of such tuples. Memory activation of the memory instance $i$ is modulated by at least two processes (i.e., free parameters in the model): memory decay and noise associated with the retrieval of these memories. At time step $t$, let there be $n < t$ unique memory instances in memory and suppose a new state $s_t$ is encountered at the current time $t$, then the activation score $A_i(t) $ of memory instance $i$ $(s_i, a_i, u_i)$, is given by: 
%
%\begin{equation}
%A_{i,t} = \ln \; \sum_{j = 1}^{n_i} (t_j)^{-d} + \mu \sum_{k=1}^K \mbox{Sim}(s_{i,k}, s_k) +  \epsilon
%\label{eq: activation}
%\end{equation}
{\small 
\begin{align}
\ln \big(  \sum_{t' \in \mathcal{T}_i(t)} (t - t')^{-d}\big) +  \mu \sum_{j =1}^K \omega_j Sim(s_{i,j},s_{t,j}) + \sigma \xi 
\label{eq:activation}
\end{align}
}
%
where $d$ is a decay parameter, $\mathcal{T}_i(t)$ is the set of time steps of occurrence of instance $i$ in memory before time $t$, Sim is a domain specific similarity function with range in $[0,1]$, $\mu, \omega_j > 0$ are weights (typically $1$), and noise $\sigma \xi$ introduces stochasticity in retrieval and it is a $\sigma$ scaled random variable $\xi$ with zero mean logistic distribution.
The activation score of each instance in memory determines its retrieval probability. Consider an action $a$ and the set of all instances in memory with action $a$ as $M_a$.
The retrieval probability is calculated for each instance $i \in M_a$ using the Boltzman softmax function $P_{i,t} = \frac{e^{A_{i}(t)/\tau}}{\sum_{j \in M_a} e^{A_{j}(t)/\tau}}$ and then the model chooses the action $a^*$ with the highest \textit{blended} value \textit{V}:
{\small
\begin{equation}
V_{t}(a) = \sum_{i=1}^{|M_a|}P_{i,t}u_i \; , \; a^* = \arg\!\max_{a \in A} V_{t}(a)
\label{eq:prob_retrieval} 
\end{equation}
}
% 
where $\tau$ is a temperature parameter with a default value of $\tau=\sigma\sqrt{2}$. We note that the \emph{blending} operation here is exactly like 
the soft attention weighted retrieval in modern deep learning but the blending concepts in cognitive science (IBL and ACT-R) predate these modern notions. Blending concepts are themselves inspired by similar ideas present in early AI literature~\citep{gonzalez2003instance}. Another concept used in IBL is called \emph{tracing} ~\citep{Cranford2020,Lebiere2023} inspired from feedback in intelligent tutoring systems~\citep{Anderson95}. When tracing, the model fills the memory using the true ground memory instances due to the human participant action and outcome for each new prediction, instead of the model using its own prediction and outcome. This process enables the model to anticipate the next-trial decision and align the model's memory with the participant's specific experience. This aspect is analogous to teacher forcing~\cite{williams1989learning} in recurrent neural networks in AI literature.
The connections of IBL to AI concepts inspired us to explore modern neural network techniques, as described next.



%For three of the features of the model, namely payment, penalty, and monitoring probability, we have added the following similarity functions:
%\begin{equation} \label{eq:payment_penalty} 1 - \frac{\left| x - y \right|}{10} \end{equation}
%\begin{equation} \label{eq:Mprob} 1 - \left| x - y \right| \end{equation}


\subsection{Token-Level Model}
Pretrained on extensive datasets, LLMs have demonstrated significant potential in tasks such as text generation and semantic analysis. Prior works~\cite{} have found that finetuning a pretrained LLM enhances its ability to address new problems effectively. Following IBL model, we incorporate personalized memory into the LLM, where this memory comprises a sequence of memory instances. This approach is called Token-Level Personalized Memory Integrated Model (TL-PMIM). This approach is implemented by integrating the memory into the context. Mathematically, we concatenate the instance sequences in the memory with the current situation as the input $s_t$ and construct the input-output pair $(x_t, a_t)$ where $x_t$ is: 
\begin{equation*}
    x_t = s_1 || a_1 || u_1 \ldots s_{t-1}|| a_{t-1} || u_{t-1} || s_t
\end{equation*}

We then fine-tune an LLM with the dataset $\mathcal{D}=\{(x_t, a_t)\}^N_{i=1}$. A concrete input example is provided in the appendix. 

\subsection{Instance-Level Model}
While the TL-PMIM offers substantial model expressivity, it is associated with higher computational costs and reduced interpretability. To address these issues, we propose the Instance-Level Personalized Memory Integrated Model (IL-PMIM), which balances expressivity and interpretability through a simple attention-layer-based architecture. The simple attention-layer provides a direct interpretation of importance in terms of the learned attention weights. 
Similar to TL-PMIM and IBL, the memory is a sequence of memory instances. However, IL-PMIM introduces an additional processing step. Specifically, each memory instance $(s,a,u)$ is encoded into two latent vectors by a text encoder $E$. One latent vector represents the state and utility, denoted by $e^{s,u}$, and the other representing the action, denoted by $e^a$. The attention layer then processes this sequence of encodings along with the encoding of the current state to produce the action for the current step. We note the choice of producing two encoded vectors per memory instance is a trade-off: using a single latent vector for a memory instance led to the attention ignoring the action probably because likely the action information was lost in the encoding. On the other hand, using three separate encoded vectors for state, action, and utility leads to a long memory sequence which is not processed well by the simple attention layer.  Mathematically, IL-PMIM can be expressed as follows: 


\begin{align}
    & e^{s,u}_i = E(s_i || u_i)\;,\;
    e^a_i = E(a_i) \text{ for } i<t-1\;, \;
    e^s_t =E(s_t) \;, \quad 
    x_t = (e_1^{s,u}, e_1^a, \ldots, e_{t-1}^{s,u}, e_{t-1}^a, e^s_t) \nonumber \\
    & \hat{a}_{t} = f_\theta(\sum_{j=1}^{2t-1} A_j V_j) \;\mbox{ where } \; \{A_j\}_{j=1}^{2t-1}, \{V_j\}_{j=1}^{2t-1} = Att_w(x_t) \label{eq:attention}
\end{align}

where $f_\theta$ is a multilayer perception that outputs the predicted action $\hat{a}_{t}$ and $Att_w$ is a simple attention layer with $w$ the weights of the query, key, and value transformation from each component of $x_t$. 


% \subsection{Decoder-Only Behavior Imitating} 
% We exploit the powerful pretrained LLMs and finetune it to mimic the human's behavior. As we would like to learn the human's preference from only their history decisions, we have designed the memory mechanism. The input of the LLM consists of all history emails, decisions,  feedback (if exist), and the current email, while the output of the LLM is the predicted decision that a human with the given memory may make. 

% We would like to remark that this approach can fully utilize all the training data while it still learns the preference of each human by the special design of the memory mechanism. 

% \subsection{Hybrid Approach} 
% Instead of training a model at the token level such as our decoder-only behavior imitating approach, we propose an alternative approach that trains the model at the email level. 

% In this approach, we embed the emails and decisions by the encoder-decoder language model. We then apply a shallow transformer to process the embedding sequences and to output the predicted decision.

% The input of the model consists of a sequence of embeddings, which contain the information of the history emails and the current one. According to our initial investigation, we choose to embed the email content and the human's decision of the email separately. We obtain these embeddings by the encoder-decoder language model, embedding of $x_i$ denoted by $e^x_i$ and embedding of $a_i$ denoted by $e^a_i$. The input can be represented by $(e^x_1, e^a_1, e^x_2, \ldots, e^x_t)$. 

\subsection{GPT3.5 Approach} \label{sec:gptdesc}
We also experiment the zero-shot performance of LLMs as cognitive models. Similar to the TL-PMIM model, the GPT3.5 model is incorporated with a personalized memory module. Due to cost reasons, we cannot pass the entire memory in the prompt hence we process the memory to retrieve the top $k$ instances. Let $s_t$ be the current email in consideration, then each instance in the memory $(s_i, a_i)$ for $i \in [1, t-1]$ is given a score $Sim(s_i, s_t)$, where $Sim$ is a domain specific similarity function. The top $k$ instances ${s_i, a_i}$  are then retrieved to create the input $x_t$ as, 
\begin{equation*}
    x_t = s_1 || a_1 || u_1 \ldots s_{k} || a_{k} || u_{k} || s_t
\end{equation*}
The LLM is then prompted to provide action $a_t$. Note that the full prompt also contains additional information such as task description and an in-context example to help the LLM. It is also asked to provide a justification for its decision to ensure that the LLM uses the memory to make the decision vs its own prior knowledge. An example of the prompt and justification given by the LLM is provided in the appendix.

==> sections/4_exp.tex <==
\section{Experiments}\label{sec:exp}
The experiments are designed to evaluate if our approach can model the human responses with high fidelity, i.e., decision pattern of our model is similar to that seen in the data. For TL-PMIM, we have fine-tuned Llama 2 7B base using LongLora~\citep{longlora}. For the encoding $E$ in IL-PMIM we use a sentence transformer, namely all-mpnet-base-v1~\citep{all-mpnet-base-v1}.

We consider two baselines from literature. One is the IBL model~\citep{cranford2019modeling,cranford_towards_2021}.  Another is the direct use of the GPT3.5 model. 
 All neural network experiments were run on NVIDIA Quadro RTX 5000 GPUs except for TL-PMIM, which was run on NVIDIA H100 GPUs. Hyperparameters for TL-PMIM are constant learning rate 2e-5 with a warmup of 20 steps, batch size 32, 1 training epoch with AdamW optimizer. Hyperparameters for IL-PMIM are constant learning rate $5e$-$6$ with a batch size of $64$ and a dropout of $0.1$. The key, query and value embedding dimensions are $256$. The model is trained for $1000$ epochs with an Adam optimizer.

\subsection{Domain and Data}

We explore two dynamic decision-making domains in this work. The two domains chosen require somewhat varying skills: one requires visual and memory skills to detect phishing email, the other requires quantitative risk assessment skills to decide the best course of action.  Data for both these domains were obtained from human subject experiments in prior works. We describe the human subject experiment from past work in brief and also the data gathered from these experiments below.

\textbf{Phishing Dataset}: We use the Phishing dataset from~\cite{singh2019training}. The data is collected from the human participants in human subject experiment. The experiment had three phases: pre-training, training, and post-training. Each participant received 10 emails in pre- and post-training phase respectively, while they received 40 emails in the training phase. The 10 post-training emails (2 phishing, 8 ham) were deliberately chosen from a different distribution to test out of distribution response. For every email, they are asked to answer if the email is phishing or ham. These emails were selected from a pool of 239 emails, encompassing both legitimate (ham) and phishing emails.
The dataset had data of 297 participants. Three groups (same size) of participants receives three different percentage of training emails that were phishing emails: 25\%, 50\%, and 75\%. In addition to this data, we also have auxiliary data which provide six binary labels for every email used in the study. These labels are from domain experts and characterize why the email is phishing or not. The label names are self-explanatory: (1) sender mismatch, (2) request credentials, (3) subject suspicious, (4) asks to do something urgently, (5) has some offer(s), and (6) mismatch in link text and location. We do not use this auxiliary data in training but use them for evaluation of our model.

The email information is the state for our memory instance; this state data has the sender, subject and body of email represented in words. The action is binary: yes or no for phishing. The utility is 0 or 1 based on correct detection of phishing or ham. To investigate the effects of the data size on training of our models, we split the dataset in two ways. In the first way, the first 10 emails are used for training while the remaining 50 emails are used for testing (10:50 split). In the second way, the first 50 emails are used for training while the last 10 emails are used for testing (50:10 split). 

As stated in earlier sections, we need similarity scores between emails. In IBL, we followed a prior work~\citep{xu2022modeling} where cosine similarity was computed on BERT embeddings. For GPT, we used an embedding tool from~\cite{ni2021large} to embed emails and then used cosine similarity.

\textbf{IAG dataset}:  The Insider Attack Game (IAG) is designed as an online game that simulates real-world scenarios in the lab such as in~\cite{cooney_learning_2020}. It involves two stages: first, defenders protect nodes (computers) by a randomized allocation of limited resources and the attacker chooses a node to attack. In the second stage, the defender chooses probabilistically to either warn the attacker that the node is defended (which could be a lie) or not provide such warning, and then the attackers choose to continue the attack or not. The defender's defense and deceptive strategies are decided based on prior work in Stackelberg games~\citep{xu2015exploring}. The game has six nodes (computers), with the resource constrained defender able to protect only two.

 In the human subject study, participants acted as insider attackers, aiming to gain points by attacking nodes. Attackers earn points if the node they attack is undefended but lose points if caught. The exact number of points depends on the node, ranging from -10 to +10. If an attacker decides to withdraw the attack in the second stage, they don't earn any points. Here, we aim to model the second stage decision of the human participant, i.e., whether to continue the attack or not. The decision to continue attack is optimal if the ground truth status of the node is uncovered (undefended) and not optimal if the node is covered.
We obtain the dataset from~\cite{aggarwal_deceptive_2023}. The dataset had information about which node was chosen (target number, target location), the probability of the node being defended, the reward (or penalty) points if the node was undefended (or defended), the actual defended or not status of the node, and the outcome expressed in the number of points obtained by the participant based on his decision to continue attack or not. In the dataset, participants played the game 100 times each for different settings (different node points, defender strategy, etc.) for a total of 107900 game instances played. Given the larger number of data points (than phishing dataset) we perform a 50\% split for training and testing for the IAG dataset.

As stated in earlier sections, we need similarity scores between the state features. In IBL, we followed the approach in prior work~\cite{cranford_learning_2018,nguyen_speedyibl_2023} where a similarity is computed for each feature and then summed over the features. For both reward and penalty features the similarity is $1 - \frac{\left| x - y \right|}{10}$ and for the probability of defended feature the similarity is $1 - \left| x - y \right|$. For other features (target number, target location, and defended) an exact
match is $1$ or else $0$.
For GPT, we used the same similarity score to trim the prompt, as described earlier in Section~\ref{sec:gptdesc}.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.\textwidth]{img/section-4.1.1/no_cat/phishing-5010/confusion_matrix.png}
    \caption{Phishing confusion matrix with 50:10 split}
    \label{fig:phish5010}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=1.\textwidth]{img/section-4.1.1/no_cat/phishing-1050/confusion_matrix.png}
    \caption{Phishing confusion matrix with 10:50 split}
    \label{fig:phish1050}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=1.\textwidth]{img/section-4.1.1/no_cat/iag/confusion_matrix.png}
    \caption{IAG confusion matrix}
    \label{fig:iag}
\end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\textwidth]{img/memo-enabled model.jpg}
%     \caption{Illustration of the Memory Module}
%     \label{fig:memo-gen}
% \end{figure}

\subsection{Evaluation and Comparison}



\textbf{Aggregated Results}:
We show the average test performance (accuracy of matching the human decision) of the models under consideration in Figures~\ref{fig:phish5010},~\ref{fig:phish1050}, and~\ref{fig:iag}. It can be seen that the performance of TL-PMIM and IL-PMIM drops in the phishing domains when the amount of training data is lower. Supporting this trend, their performance are much better in the high data IAG domain. IBL seems to have similar performance overall, possibly due to limited model capacity. GPT does not suffer much in low data domain, possibly due to a much richer prior knowledge base inbuilt into the GPT3.5 model.

In more details, we see the average (across participants) performance of the models over each trail in the test set in Figure~\ref{fig:overtrials}. For phishing emails, in the 10:50 split we see a drop in performance of all models, except IBL, staring in the 51st trial. This is due to the change in distribution of emails for the last 10 post-training emails, as stated in the data description. IBL does not suffer a drop in this case, likely because of its low capacity leading to better out of distribution performance. 





% \begin{figure}[h]
%   \centering
%   \begin{subfigure}[b]{0.315\textwidth}
%     \includegraphics[width=\textwidth]{img/section-4.1.1/no_cat/phishing-1050/accuracy_over_time.png}
%     \caption{Caption for second figure}
%     \label{fig:subfig2}
%   \end{subfigure}
%   \hspace{0.01\textwidth}
%   \begin{subfigure}[b]{0.315\textwidth}
%     \includegraphics[width=\textwidth]{img/section-4.1.1/no_cat/phishing-5010/accuracy_over_time.png}
%     \caption{Caption for first figure}
%     \label{fig:subfig1}
%   \end{subfigure}
%   \hspace{0.01\textwidth}
%   \begin{subfigure}[b]{0.315\textwidth}
%     \includegraphics[width=\textwidth]{img/section-4.1.1/no_cat/iag/accuracy_over_time.png}
%     \caption{Caption for third figure}
%     \label{fig:subfig3}
%   \end{subfigure}
%   \caption{Overall caption for the three figures}
%   \label{fig:subfigures}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{img/section-4.1.1/no_cat/acc-over-time.png}
    \caption{Model human alignment over trials in the test set. (Left) Phishing with 10:50 split; (Middle) Phishing with 50:10 split; (Right) IAG}
    \label{fig:overtrials}
\end{figure}


\textbf{Prediction accuracy increases with Human's Accuracy}:
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{img/section-4.1.1/by_human_acc/combined.pdf}
    \caption{Model performances split by human's accuracy (Left) Phishing 50:10, (Center) Phishing 10:50, (Right) IAG }
    \label{fig:splitground}
\end{figure}
Next, we split the results by how accurate is the human prediction of the ground truth, which in phishing domain is whether the email was actually phishing or not and in IAG whether it was optimal to continue the attack or not. We split the model-human decision synchronization result by the accuracy of the ground truth prediction by human and show the results in Figure~\ref{fig:splitground}. The number of participants in each bucket in the figure is roughly the same. We notice that when there is sufficient data (phishing 50:10 or IAG) the models generally do better when the human decisions align with the ground truth. This is not true for GPT which has similar performance in most scenarios, suggesting that it relies on its prior knowledge more than trying to mimic the human's observed performance. 

Further, for the phishing 10:50 split TL-PMIM shows improvement similar to the sufficient data scenario; this further suggests that fine-tuning a LLM helps in better mimicking human behavior, especially when the human behavior exhibits learnable patterns such as being able to detect phishing email. We also conjecture that when the human does not predict the ground truth well, then there may not be one pattern of mistake but a mix of variety of suboptimal behavior by a single human. This is likely why for low data domain of phishing (per participant) the performance at lower human accuracy is much worse than in the high data domain of IAG. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{img/section-4.1.1/by_ph_rate/combined_rate.pdf}
    \caption{Model performances split by \% of phishing (Left) Phishing 50:10, (Right) Phishing 10:50}
    \label{fig:percentagephish}
\end{figure}


\textbf{More Fine-grained Analysis}:
We look at more fine-grained results here for the phishing domain. We present yet more fine-grained results in the appendix where we look at the results split by different labels of ground truth. 

Figure~\ref{fig:percentagephish} shows the results in the phishing domain split by participants who see different percentages of phishing emails in training. All models, except GPT, do slightly better in 50:10 split for those participants that see fewer phishing emails, given we observed that overall human accuracy (of detecting phishing and ham emails) is slightly higher when they see fewer phishing emails. The variance across the different percentage groups is minimal for the 10:50 split. %{\color{blue}WHY???}


\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
\includegraphics[width=\linewidth]{img/section-4.1.1/retrieval_feature_matching/retrieval_feature_matching.pdf}
    \caption{Average similarity between the six auxiliary features of the current email to the top ranked emails in the memory and bottom ranked emails in the memory.}
    \label{fig:cosine}
\end{wrapfigure}

Next, we look at which emails in memory do the interpretable models IBL and IL-PMIM pay attention to when deciding about the next email $e_0$. In particular, we can extract the relevance of emails in memory for IBL using the retrieval probability defined in Equation~\ref{eq:prob_retrieval}. For IL-PMIM we can do the same using the attention weights defined in Equation~\ref{eq:attention}. Then, we rank the emails in memory and extract the top five relevant ones $R$ and bottom five relevant ones $N$. Recall from the phishing data description, that for every email $e$ we have an auxiliary vector $v_e$ of size six, denoting the presence or absence of characteristics that make the email a phishing email or not. Then, we compute the $(1/5)\sum_{e \in R} Sim(v_{e_0}, v_e)$ and $(1/5)\sum_{e \in N} Sim(v_{e_0}, v_e)$ where $Sim$ is cosine similarity. These numbers measure how relevant the top five and bottom five emails are to the current email from the perspective of phishing characteristics.  We expect to see a difference between these two numbers, which is what we show in Figure~\ref{fig:cosine}. The figure show the results split by ground truth phishing or ham email and shows that IL-PMIM and IBL have roughly the same degree of attention difference between the top and bottom five case. Next, we note that TL-PMIM is not interpretable by design, and while there is a lot of work on explaining transformer outputs, the explainability tools generally have no guarantee. We also found that these do not scale to the size of our Llama 7B model with some of the longer context lengths. Nonetheless, we provide some qualitative results next for TL-PMIM.



\textbf{Qualitative Results}:
We show a qualitative result for TL-PMIM given by an interpretability tool~\cite{achtibat2024attnlrp} for a phishing email (with small memory length of 10 instances) in the box below; this email was correctly classified by the human and the TL-PMIM matched human decision. The parts highlighted in yellow by the tool are considered important by the model, which can be considered as a proxy for what the human focuses on. In the box, we also mark (as superscript) parts of email that indicate phishing nature based on the six auxiliary labels we have for all email (this email has five characteristics). It can be seen that these marked parts are also highlighted.

\begin{tcolorbox}[colback=white!10, colframe=black, title=Interpretability tool~\cite{achtibat2024attnlrp} output]
{\small
Sender: accounts@\hl{paypal.security.com}$^5$ \\
Subject: \hl{Un}autho\hl{rized Account Access Attempt}$^1$ \\
Body: \hl{Potential} Unauthorized Account Access \hl{Attempt!} \hl{Case id} : 9000321-128. \hl{Login attempt} from \hl{unknown} device. \hl{Date:} 1/\hl{25/2017} \hl{Time: 12}:00 \hl{PM} EST \hl{Dear Client On 1/25/2017} an attempt was made to access your account from an unknown \hl{IP Address} (54.875.24.152). In an \hl{effort} to protect your personal and financial \hl{information we have temporarily}$^2$ locked your account. This \hl{includes} the ability to withdrawl funds. The access attempt was blocked prior to the unauthorized individual (or individuals) gaining access so, at this time, \hl{your} personal and \hl{financial} information remains secure. If \hl{this} attempt was made by you, or you \hl{authorized} the third party access, \hl{we} apologize for the inconvenience. However, in order to unlock your account and protect the \hl{integrity} of your personal and financial \hl{information}, you \hl{must} pass a security check. Also note that this is a \hl{time sensitive} matter. You \hl{must} complete the security check \hl{within 72 hours}$^2$ of the \hl{date} of this \hl{email}. Should you choose not to \hl{comply, your} account \hl{will} be \hl{permanently locked} and any funds contained therein will be forfeited. To \hl{begin, please: 1. Right click on}$^3$ the \hl{link PayPal Member Security Services}$^3$ 2. \hl{Open} the \hl{page} in a \hl{secure (private) browser window}. 3. Follow the instructions provided. \hl{Please} note \hl{that PayPal} will never ask for your \hl{password}$^4$ over the phone, nor ask you to send your login credentials via email. \hl{Don't wait}$^2$. \hl{Protect} your information and unlock your account within the \hl{next 72 hours to}$^2$ avoid the \hl{loss} of \hl{your} account and \hl{forfeiture of funds}. \\

Expert Labels: \\
$1:$ Subject suspicious \\
$2:$ Asks to do something urgently \\
$3:$ Mismatch in link text and location \\
$4:$ Requests Credentials \\
$5: $ Sender Mismatch 
}
\end{tcolorbox}

% \begin{table}[htbp]
%     \centering
%     \caption{Model Comparison}
%     \label{tab:model_comparison}
%     \begin{tabular}{lcc}  % Adjust column alignment as needed (left-aligned 'l', center-aligned 'c', right-aligned 'r')
%         \toprule
%         \textbf{Model} & \textbf{Data} & \textbf{Accuracy (\%)} \\
%         \midrule
        
%         \multirow{3}{*}{Hybrid} 
%                                 & 10:50 & 48.7 \\
%                                 & 30:30 & 62.1 \\
%                                 & 40:20 & 62.9 \\
%                                 & 50:10 & 60.1 \\
%         \cline{1-3} % Horizontal line after merged rows
%         \multirow{5}{*}{Fine-Tune} 
%                                 & 10:50 & 61.6 \\
%                                 & 20:40 & 63.7 \\ 
%                                 & 30:30 & 73.3 \\
%                                 & 40:20 & 74.5 \\
%                                 & 50:10 & 72.3 \\
%         \cline{1-3} % Horizontal line after merged rows     
%         \multirow{5}{*}{IBL} 
%                                 & 10:50 &  \\
%                                 & 20:40 &  \\ 
%                                 & 30:30 &  \\
%                                 & 40:20 &  \\
%                                 & 50:10 &  \\
%         \cline{1-3} % Horizontal line after merged rows     
%         \multirow{3}{*}{GPT-3.5} 
%                                 & 30:30 & 65.2\\
%                                 & 40:20 &  \\
%                                 & 50:10 &  \\
%         \bottomrule
%     \end{tabular}
% \end{table}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\textwidth]{img/acc_over_time-3030.png}
%     \caption{Accuracy over number trials with train-test split of 30:30}
%     \label{fig:acc_time-3030}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\textwidth]{img/acc_over_time-4020.png}
%     \caption{Accuracy over number trials with train-test split of 40:20}
%     \label{fig:acc_time-4020}
% \end{figure}

==> sections/5_limit.tex <==
\section{Limitations, Future Work, and Broader Impact}\label{sec:limit}

Our work aims to show how neural networks can aid in improving cognitive modeling of dynamic decision-making.
We note some limitations and potential impact of our approach. First, we have shown our results only on two tasks with data collected in a structured lab setting. Even though the tasks are quite distinct, more validation of our results can be achieved by analyzing tasks in the real world. For example, when detecting phishing emails in an office setting, humans many be juggling many other tasks and hence factors such as time available to make the decision becomes important; these have sometime been considered in cognitive science~\citep{kerstholt1995decision}. It is always possible to expand our neural network based models with these additional factors (if measured and recorded) but such a work is beyond the scope of a single paper.
Next, one of the core advantages of the prior popular IBL model is interpretability. However, our black box TL-PMIM model mimics the dynamic decisions with higher fidelity than IBL without having explanations for all predictions. This is because computing reasonable explanations for LLMs is currently very computationally expensive. %This raises basic questions about whether models of human cognition should be interpretable given that the human brain is so complex. 
Without some degree of explanation, we cannot be assured of neural networks not learning spurious correlations. Thus, there is a need to explain LLMs with large context lengths in a scalable manner.
%This points to promising direction where models like TL-PMIM can be used to expand the elements of cognition in behavioral science literature to be able to explain and match TL-PMIM. 
 Finally, while our work is geared towards creating positive social impact by ultimately designing interventions to make humans detect phishing better or understand attacker strategy to design better cyber-defense, there are potential issues to be wary of. Any model of human behavior can be used by attackers to try and improve their attacks (e.g., create phishing email) to bypass detection more successfully.  We caution against the use of our methods without appropriate checks and guardrails. 

 Overall, our work has shown that there is positive synergy to be gained from bringing together concepts from modern deep learning and human cognition sciences; we envision neural networks being adopted in cognitive sciences for higher fidelity behavior modeling and possibly concepts from cognitive sciences leading to newer specialized neural network architectures.
 
 %Further, sometimes human behavior analysis tools have been used for unintended purpose, such as in job interviews, but trained on very non-diverse data.
 %But, we also would like to point out that security is a cat and mouse game and our aim to be more secure cannot rely on the attacker not possessing advanced models. 

==> sections/6_conclusion.tex <==
\section{Conclusion}
